On the cohomology rings of tree braid groups

Let $\Gamma$ be a finite connected graph. The (unlabelled) configuration space $UC^n \Gamma$ of $n$ points on $\Gamma$ is the space of $n$-element subsets of $\Gamma$. The $n$-strand braid group of $\Gamma$, denoted $B_n\Gamma$, is the fundamental group of $UC^n \Gamma$. We use the methods and results of our paper "Discrete Morse theory and graph braid groups" to get a partial description of the cohomology rings $H^*(B_n T)$, where $T$ is a tree. Our results are then used to prove that $B_n T$ is a right-angled Artin group if and only if $T$ is linear or $n<4$. This gives a large number of counterexamples to Ghrist's conjecture that braid groups of planar graphs are right-angled Artin groups.

==> bibs <==
\begin{thebibliography}{10}

\bibitem{Abrams}
Aaron Abrams.
\newblock {\em Configuration spaces of braid groups of graphs}.
\newblock PhD thesis, UC Berkeley, 2000.

\bibitem{BridsonHaeflinger}
Martin~R. Bridson and Andr{\'e} Haefliger.
\newblock {\em Metric spaces of non-positive curvature}, volume 319 of {\em
  Grundlehren der Mathematischen Wissenschaften [Fundamental Principles of
  Mathematical Sciences]}.
\newblock Springer-Verlag, Berlin, 1999.

\bibitem{Brown}
Kenneth~S. Brown.
\newblock The geometry of rewriting systems: a proof of the
  {A}nick-{G}roves-{S}quier theorem.
\newblock In {\em Algorithms and classification in combinatorial group theory
  (Berkeley, CA, 1989)}, volume~23 of {\em Math. Sci. Res. Inst. Publ.}, pages
  137--163. Springer, New York, 1992.

\bibitem{CharneyDavis}
Ruth Charney and Michael~W. Davis.
\newblock Finite {$K(\pi, 1)$}s for {A}rtin groups.
\newblock In {\em Prospects in topology (Princeton, NJ, 1994)}, volume 138 of
  {\em Ann. of Math. Stud.}, pages 110--124. Princeton Univ. Press, Princeton,
  NJ, 1995.

\bibitem{ConnollyDoig}
Frank Connolly and Margaret Doig.
\newblock {Braid groups and right angled Artin groups}.
\newblock {\em arXiv:math.GT/0411368}.

\bibitem{CrispWiest}
John Crisp and Bert Wiest.
\newblock Embeddings of graph braid and surface groups in right-angled {A}rtin
  groups and braid groups.
\newblock {\em Algebr. Geom. Topol.}, 4:439--472, 2004.

\bibitem{Dugundji}
James Dugundji.
\newblock {\em Topology}.
\newblock Allyn and Bacon Inc., Boston, Mass., 1966.

\bibitem{Farber2}
Michael Farber.
\newblock {Collision Free Motion Planning on Graphs}.
\newblock {\em arXiv:math.AT/0406361}.

\bibitem{Farber1}
Michael Farber.
\newblock Topological complexity of motion planning.
\newblock {\em Discrete Comput. Geom.}, 29(2):211--221, 2003.

\bibitem{FS1}
Daniel Farley and Lucas Sabalka.
\newblock Discrete {M}orse theory and graph braid groups.
\newblock {\em Algebr. Geom. Topol.}, 5:1075--1109 (electronic), 2005.

\bibitem{Farley2}
Daniel~S. Farley.
\newblock Homology of tree braid groups.
\newblock {\em to appear in Proceedings of the Conferences on Probabilistic and
  Asymptotic Aspects of Group Theory and Topological Aspects of Group Theory,
  Edited by: R.I. Grigorchuk, M. Mihalik, M. Sapir, and Z. Sunik}.

\bibitem{Farley1}
Daniel~S. Farley.
\newblock Homological and finiteness properties of picture groups.
\newblock {\em Trans. Amer. Math. Soc.}, 357(9):3567--3584 (electronic), 2005.

\bibitem{Forman}
Robin Forman.
\newblock Morse theory for cell complexes.
\newblock {\em Adv. Math.}, 134(1):90--145, 1998.

\bibitem{Ghrist}
Robert Ghrist.
\newblock Configuration spaces and braid groups on graphs in robotics.
\newblock In {\em Knots, braids, and mapping class groups---papers dedicated to
  Joan S. Birman (New York, 1998)}, volume~24 of {\em AMS/IP Stud. Adv. Math.},
  pages 29--40. Amer. Math. Soc., Providence, RI, 2001.

\bibitem{Gubeladze}
Joseph Gubeladze.
\newblock The isomorphism problem for commutative monoid rings.
\newblock {\em J. Pure Appl. Algebra}, 129(1):35--65, 1998.

\bibitem{Hatcher}
Allen Hatcher.
\newblock {\em Algebraic topology}.
\newblock Cambridge University Press, Cambridge, 2002.

\bibitem{Hu}
Sze-tsen Hu.
\newblock Isotopy invariants of topological spaces.
\newblock {\em Proc. Roy. Soc. London. Ser. A}, 255:331--366, 1960.

\bibitem{Mautner}
Carl Mautner.
\newblock Private communication.

\bibitem{Salvetti}
M.~Salvetti.
\newblock Topology of the complement of real hyperplanes in {${\bf C}\sp N$}.
\newblock {\em Invent. Math.}, 88(3):603--618, 1987.

\end{thebibliography}

